From Single-Agent Self-Discovery to Multi-Agent Adaptation: Scaling Laws of Partner Feedback and Convention Rigidity in Meta Reinforcement Learning Algorithms

A key milestone toward Recursive Self-Improvement (RSI) is replacing hand-crafted optimizers with meta-learned update rules (such as Disco103 and OPEN) that discover how agents learn. Yet when a self-discovered RL model trains with adapting teammates, does co-evolution sustain capability gains or trap agents in brittle conventions? Across 1,800+ runs in continuous collective robotics (VMAS) and discrete coordination (Overcooked), we establish five laws of multi-agent adaptation. First, four-cell counterfactual partner swaps expose an evaluation illusion: apparent team progress often masks focal regression (+1.066 team gain concealing -0.119 focal loss) and inflates transfer by +0.649 to +1.210. Second, a 288-run physical-coupling sweep ($\alpha \in [0, 1.5]$) reveals a linear scaling law ($\beta = +0.255$, $p = 0.000488$, Spearman $\rho = 1.0$): live reciprocal feedback keeps Disco103 invariant (AUC 0.297--0.322), whereas severing feedback triggers a monotonic collapse (-0.172 to -0.490), with OPEN establishing a sensitivity spectrum (Disco103 > OPEN > MAPPO). Third, extending navigation training eightfold (1.05M steps) enables Disco103 to overtake MAPPO (+0.087 team return, +0.133 bank gain), while decoupled training boosts cross-partner completion by +10.16% (56.25% vs. 46.09%). Fourth, in Overcooked, MAPPO's self-play conventions induce a 28.13% cross-partner collision rate, whereas Disco103 cuts collisions to 12.77% and achieves 3.33x higher bank return (9.96 vs. 2.99; net gain +6.43), further improved by decoupled meta-adaptation (+1.39 with scripted partners). Finally, perturbation pulses ($p=0.00098$), auxiliary entropy diagnostics (8.485 nats), and 48 multi-lifetime meta-evolved rules ($L_2 \in [2.11, 4.91]$) trace these dynamics to partner-gradient blindness and auxiliary drift, informing multi-agent self-discoverd algorithms.

==> fonts/arial-setup.tex <==
\pdfmapfile{+fonts/arial.map}
\DeclareFontFamily{T1}{labarial}{}
\DeclareFontShape{T1}{labarial}{m}{n}{<-> fonts/arialregular}{}
\DeclareFontShape{T1}{labarial}{m}{it}{<-> fonts/arialitalic}{}
\DeclareFontShape{T1}{labarial}{m}{sl}{<-> fonts/arialitalic}{}
\DeclareFontShape{T1}{labarial}{b}{n}{<-> fonts/arialbold}{}
\DeclareFontShape{T1}{labarial}{bx}{n}{<-> fonts/arialbold}{}
\DeclareFontShape{T1}{labarial}{b}{it}{<-> fonts/arialbolditalic}{}
\DeclareFontShape{T1}{labarial}{bx}{it}{<-> fonts/arialbolditalic}{}

